GIM: Gaussian Isolation Machines

In many cases, neural network classifiers are likely to be exposed to input data that is outside of their training distribution data. Samples from outside the distribution may be classified as an existing class with high probability by softmax-based classifiers; such incorrect classifications affect the performance of the classifiers and the applications/systems that depend on them. Previous research aimed at distinguishing training distribution data from out-of-distribution data (OOD) has proposed detectors that are external to the classification method. We present Gaussian isolation machine (GIM), a novel hybrid (generative-discriminative) classifier aimed at solving the problem arising when OOD data is encountered. The GIM is based on a neural network and utilizes a new loss function that imposes a distribution on each of the trained classes in the neural network's output space, which can be approximated by a Gaussian. The proposed GIM's novelty lies in its discriminative performance and generative capabilities, a combination of characteristics not usually seen in a single classifier. The GIM achieves state-of-the-art classification results on image recognition and sentiment analysis benchmarking datasets and can also deal with OOD inputs.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Regularization.tex <==
In this section, we examine the effectiveness of using Equations \eqref{eq3} and \eqref{eq4} as regularization terms, along with the cross-entropy loss function. The purpose of these regularization terms is to limit, to some extent, the hypothesis space. The regularization terms are applied to the logits, denoted by $z$, i.e., the input to the softmax activation. The $CTV(c)$ and the $CH(c)$ terms are also calculated using the logits and not the output of the neural network.
\begin{figure}[th]
\centerline{
\includegraphics[scale=0.36]{Figures/LogitsMargin.png}}
\caption{MNIST classification: class 1 vs class 2 logits space}
\label{figure6}
\end{figure}
The regularization will limit the logits of each class to a cluster form if Equation \eqref{eq3} is used then, or to a sphere in cases where Equation \eqref{eq4} is used.
We a show a visualization to convey the intuition we had for making CVC regularization in Figure~\ref{figure6}.
The regularization forces a large margin relatively to the scatter's scale in the logits space. We hypothesize that the large margin effect along with narrowing the hypothesizes space is what improves the neural network's performance.
\par
We reformulate the relevant equations using the logits of the neural network, and define the regularization terms:
\begin{equation}
     CTV(c) = \frac{1}{|c|} \sum_{z\in c} \Vert \mu_{c}-z \Vert_{2}^{2}
     \label{eq12}
\end{equation}

\begin{equation}
     CH(c) = \frac{1}{|c|} \sum_{z\in c}(CTV(c)- D(z,c))^{2}
     \label{eq13}
\end{equation}
\newline
First moment regularization:
 \begin{equation}
      -\frac{1}{M}\sum_{i=1}^{M}\sum_{c\in C}y_{i,c}\log(\hat{y}_{i,c}) + 
      \frac{\lambda}{|C|}\sum_{c\in C} CTV(c)
     \label{eq14}
 \end{equation}
\newline
Second moment regularization:
 \begin{equation}
      -\frac{1}{M}\sum_{i=1}^{M}\sum_{c\in C}y_{i,c}\log(\hat{y}_{i,c}) + 
     \frac{\lambda}{|C|}
     \sum_{c\in C}CH(c)
     \label{eq15}
 \end{equation}

Because both of these terms control the variance inside each class, we refer to these regularization terms as Class Variance Control (CVC).
We evaluated our regularization methods and compared them to networks with dropout~\cite{hinton2012improving} regularization and/or $l_{2}$ weight regularization.
In the experiments, we used the architectures presented in Table~\ref{table1} and for CIFAR10 we have used ResNet20v1. For the networks with CVC regularization, we removed all other types of regularization.
In Table~\ref{table5} we present the results, which are averaged over five runs.The results presented in Table~\ref{table5} show that using CVC regularization improves the classification ability of neural networks. Both of the CVC regularization techniques are relatively easy to implement and do not increase training time compared to other forms of regularization. In the version presented, CVC is comparable to other regularization techniques that were shown to be beneficial~\cite{hinton2012improving, Tripathi2014ASO}.
This proves that regularization on the representation can be as effective as regularizing the weights directly. We expect that with further research this approach can be improved even further. \begin{table}[t]
\caption{Class Variance Control Regularization vs Standard Neural Networks with Regularization}
\begin{center}
\resizebox{0.95\textwidth}{!}{\begin{minipage}{\textwidth}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Dataset}&\multicolumn{3}{|c|}
{\textbf{CVC vs Standard }} \\
\cline{2-4} 
& \textbf{\textit{First Moment Reg}}& \textbf{\textit{Second Moment Reg}}&
\textbf{\textit{Standard}} \\

\hline
MNIST& 99.15 & \textbf{99.18} & 99.08 \\
\hline

\hline
FASHION& \textbf{93.55} & 93.15 & 93.5 \\
\hline

\hline
IMDB& \textbf{89.90} & 89.59 & 89.5 \\
\hline

\hline
CIFAR10& 91.73 & \textbf{91.83}&  91.2\\
\hline


\multicolumn{4}{l}{}
\end{tabular}
\label{table5}
\end{minipage}}
\end{center}
\end{table}


==> Unused_text.tex <==
% in each layer, s.t. the deepest the  representation; the more useful information about the input it contain. \asaf{not clear. please rephrase and add reference.}

% Yet, there are still papers that use SVMs~\cite{boser1992training} like calcification layers instead of Softmax based ones, such as~\cite{sokolic2017robust, liu2016large}. The idea behind the replacement of the Softmax is to force a wide decision boundary. But, in general, it is believed that the networks can learn sufficient solutions without regularizing the solution form itself, as in the case of Softmax classification. \asaf{the flow is not clear. there is no good connection between the previous sentence and this one. } \guy{better ? or maybe remove completely ?}


% The Softmax Classification layer rule is to give probabilistic interpretation to the outputs of the neural network~\cite{dunne1997pairing}.
% \asaf{add here a short explanation on what Softmax is with a reference.}\guy{Fixed}

%The task of data classification has been around for a long time. 
%Although methods vary from rule-based solutions to sophisticated probabilistic algorithms, it seems like there is no unified solution. 

% Deep neural networks are built by stacking up simple non-linear transformation on top of each other. Those simple non-linear transformation e.g., Relu, Softmax, Sigmoid~\cite{nwankpa2018activation}, and are parameterized by sets of weights matrices, that allows the optimization of the whole structure.
% The combination of the structured none- linear transformations together with specific domain operators like Convolution layers, Pooling layers and RNN cells, LSTM cells \cite{cnn2019survey, bengio1994learning, Pearlmutter1989LearningSS} allows the network the gradually learn local and global descriptors of the input, that forms a new representation, in which useful information can be deduced about the data distribution. 


% Although very adjustable and easy to work with,
% because of the massive amount of trainable parameters, the job of fitting the data became easy. As a result, neural networks are prone to over-fitting~\cite{},
% means of regularization have been invented, Some tries to mitigate the over-fitting effect, and most methods earthier reduce the number of updates every weight parameter is exposed to~\cite{hinton2012improving,Tripathi2014ASO}, or narrow the parameters search space~\cite{nusrat2018comparison}. Logical concepts from the past like large margin algorithms~\cite{boser1992training} and probabilistic modeling~\cite{jensen1996introduction}, that insure some level of confidence in the prediction have been forgotten.

% But with that assumption, the network lost its prediction confidence metric.


%The rest of the paper is organized as follows: In section \ref{section:two}, we review studies performed in related fields. In section \ref{section:three}, we present our proposed method for modifying, and thus improving, neural network classifiers. In section \ref{section:four}, we empirically evaluate our method and compare it to standard neural networks; in addition, we present a regularization case study, where we use part of our loss function as a regularization term for neural networks. Finally, in section \ref{section:five}, we discuss our conclusions and plans for future work.


%The neural network is trained to differentiate between the three Gaussians and is thus capable of classifying new samples based on the three classes. 
